NDP: Next Distribution Prediction as a More Broad Target

Large language models (LLMs) trained on next-token prediction (NTP) paradigm have demonstrated powerful capabilities. However, the existing NTP paradigm contains several limitations, particularly related to planned task complications and error propagation during inference. In our work, we extend the critique of NTP, highlighting its limitation also due to training with a narrow objective: the prediction of a sub-optimal one-hot distribution. To support this critique, we conducted a pre-experiment treating the output distribution from powerful LLMs as efficient world data compression. By evaluating the similarity between the $n$-gram distribution and the one-hot distribution with LLMs, we observed that the $n$-gram distributions align more closely with the output distribution of LLMs. Based on this insight, we introduce Next Distribution Prediction (NDP), which uses $n$-gram distributions to replace the one-hot targets, enhancing learning without extra online training time. We conducted experiments across translation, general task, language transfer, and medical domain adaptation. Compared to NTP, NDP can achieve up to +2.97 COMET improvement in translation tasks, +0.61 average improvement in general tasks, and incredible +10.75 average improvement in the medical domain. This demonstrates the concrete benefits of addressing the target narrowing problem, pointing to a new direction for future work on improving NTP.

==> figures/Bleu.tex <==

% 设置pgfplots参数
\pgfplotsset{
    width=0.8\textwidth, % 图表宽度
    height=0.3\textheight, % 图表高度
    grid=major, % 显示主网格
    major grid style={dotted}, % 主网格样式
    symbolic x coords={WMT22,IWSLT17,Avg.}, % x轴标签
    legend style={
        at={(0.5,1.2)}, % 图例位置
        anchor=north, % 图例锚点
        legend columns=2, % 图例列数
        column sep=2ex, % 列间距
        font=\Huge, % 图例字体大小
        inner xsep=4.4ex, 
        cells={anchor=west}, % 左对齐
        %legend cell align=left, % 确保文本和标记对齐
    },
}

\begin{tikzpicture}[scale=0.55]
    \begin{axis}[
        ybar, % 使用柱状图
        bar width=.6cm, % 减小柱状图宽度
        enlarge x limits=0.3, % 增加x轴限度
        ylabel={\Huge{BLEU}}, % y轴标签
        xtick=data, % 使用数据点作为x轴标签
        ymin=15, ymax=35, % y轴范围
        ytick={15,20,25,30,35}, % y轴刻度位置
        yticklabels={\Huge{15},\Huge{20},\Huge{25},\Huge{30},\Huge{35}}, % y轴刻度标签
        width=0.8\textwidth, % 轴宽度
        height=0.6\textwidth, % 轴高度
        ylabel style={yshift=0pt,}, % y轴标签样式
        xticklabel style={yshift=0pt, font=\Huge}, % x轴标签样式
        nodes near coords, % 在柱子上显示数字
        nodes near coords style={font=\bfseries\large}, % 设置字体加粗
        every node near coord/.append style={ color=black}, % 设置数字颜色
    ]
    % 绘制柱状图，每个模型对应一个颜色
    \addplot+ [fill=white,draw=red, area legend,postaction={pattern=north east lines,pattern color=red}] coordinates {(WMT22,17.5) (IWSLT17,23.6) (Avg.,20.6)};
    \addplot+ [fill=magenta!30,draw=red, area legend,postaction={pattern=crosshatch,pattern color=red}] coordinates {(WMT22,20.3) (IWSLT17,27.2) (Avg.,23.8)};
    \addplot+ [fill=white, draw=blue, area legend,postaction={pattern=north east lines,pattern color=blue!80}] coordinates {(WMT22,21.9) (IWSLT17,28.4) (Avg.,25.1)};
    \addplot+ [fill=cyan!30, draw=blue, area legend,postaction={pattern=crosshatch,pattern color=blue!80}] coordinates {(WMT22,24.5) (IWSLT17,31) (Avg.,27.8)};
    % 添加图例项
    \addlegendentry{T5-large(NTP)}
    \addlegendentry{T5-large(NDP)}
    \addlegendentry{T5-xl(NTP)}
    \addlegendentry{T5-xl(NDP)}
    \end{axis}
\end{tikzpicture}


==> figures/kiviat.tex <==


% Custom Kiviat diagram commands and definitions
\makeatletter
\def\tkz@KiviatGrad[#1](#2){% 
\begingroup
\pgfkeys{/kiviatgrad/.cd,
graduation distance= 0 pt,
prefix ={},
suffix={},
unity=1,
label precision/.store in=\gradlabel@precision,
label precision=0, % No decimal places
zero point/.store in=\tkz@grad@zero,
zero point=40 % Set zero point to 40
}
\pgfqkeys{/kiviatgrad}{#1}% 
\let\tikz@label@distance@tmp\tikz@label@distance
\global\let\tikz@label@distance\tkz@kiv@grad
 \foreach \nv in {1,...,\tkz@kiv@lattice}{
 \pgfmathsetmacro{\result}{35 + \nv * 5} % Start at 40 and increment by 5
 \protected@edef\tkz@kiv@gd{%
    \tkz@kiv@prefix%
    \pgfmathprintnumber[precision=\gradlabel@precision,fixed]{\result}%% used \pgfmathprintnumber instead of "\result\result"
    \tkz@kiv@suffix} 
    \path[/kiviatgrad/.cd,#1] (0:0)--(360/\tkz@kiv@radial*#2:\nv*\tkz@kiv@gap)
       node[label=(360/\tkz@kiv@radial*#2):\tiny\tkz@kiv@gd] {}; % added \tiny
      }
 \let\tikz@label@distance\tikz@label@distance@tmp  
\endgroup
}%
\makeatother

% Custom legend environment
\newenvironment{customlegend}[1][]{%
    \begingroup
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%

% Makes \addlegendimage available outside of an axis environment
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}

\definecolor{c1}{HTML}{CE93D8}
\definecolor{c2}{HTML}{ff8c1a}
\definecolor{c3}{HTML}{00aeef}
\definecolor{c4}{HTML}{B71C1C}
% Define global scale style
\tikzset{global scale/.style={
    scale=#1, % Set scaling factor
    every node/.append style={scale=#1} % Apply to every node
  }
}

\begin{tikzpicture}[
  label distance=13em, % Label distance
  global scale = 1, % Global scaling
  plot1/.style={ % Dataset 1 style
    thin, % Thin lines
    draw=c1, % Draw color red
    mark=square, % Marker shape square
    fill=c1,
    mark options={
     ball color=c1, % Marker color red
     mark size=4pt % Marker size 4pt
    },
    opacity=.5 % Opacity 0.5
  },
  plot2/.style={ % Dataset 4 style
    thin,
    draw=c2,
    mark=triangle,
    fill=c2,
    mark options={
      mark size=4pt,
      ball color=c2
    },
    opacity=.5
  },
  plot3/.style={ % Dataset 5 style
    thin,
    draw=c3,
    fill=c3,
    mark=square,
    mark options={
      mark size=4pt,
      ball color=c3
    },
    opacity=.5
  },
  plot4/.style={ % Dataset 6 style
    thin,
    draw=c4,
    mark=triangle,
    fill=c4,
    mark options={
      mark size=4pt,
      ball color=c4
    },
    opacity=.5
  }
]

\useasboundingbox (-25em,-5em) rectangle (10em,7em); % Set bounding box

\begin{scope}[scale=0.36,local bounding box=a,shift={(-12.5,0)}] % Set local scaling and position

% Define some macros for convenience
\newcommand\KivStep{0.1}
\pgfmathsetmacro\Unity{1/\KivStep}
\newcommand\zeroshift{20}

 \tkzKiviatDiagram[
   radial  style/.style ={-},
   rotate=90, 
   lattice style/.style ={black!30},
   step=\KivStep,
   gap=1,
   lattice=6,
]% 
{medmcqa,medqa,pubmedqa,careqa,AVG} % Define Kiviat diagram labels

 Draw dataset 1 Kiviat line
\tkzKiviatLine[
  plot1
](23.13889552,18.92380204,24.6,34.07400818,25.18417644)

Draw dataset 4 Kiviat line
 \tkzKiviatLine[
 plot2
 ](28.8764045,24.57973292,21.8,49.90748978,31.2909068)

 Draw dataset 5 Kiviat line
\tkzKiviatLine[
  plot3
 ](31.21922066,28.97879026,17.4,52.43373066,32.50793540)

 Draw dataset 6 Kiviat line
\tkzKiviatLine[
   plot4
 ](30.21515658,25.20816968,15.2,50.93933464,30.39066522)

% Draw graduation labels
\tkzKiviatGrad[unity=\Unity, label precision=0, zero point=\zeroshift](1)
\end{scope}

\begin{customlegend}[legend columns=2,legend style={draw=none,column sep=1ex,xshift=-9.6em,yshift=-9.5em},legend entries={model1,model 2,model 3,model4}]{(0em,-10em)}
    \addlegendimage{c1,fill=c1,mark=square,sharp plot}
    \addlegendimage{c2,fill=c2,mark=triangle,sharp plot}
    \addlegendimage{c3,fill=c3,mark=square,sharp plot}
    \addlegendimage{c4,fill=c4,mark=triangle,sharp plot}
\end{customlegend}

\end{tikzpicture}

==> figures/kurtosis.tex <==
\begin{tikzpicture}

\begin{axis}[
    name=plot1,
    ymajorgrids,
    xmajorgrids,
    grid style=dashed,
    width=.45\textwidth,
    height=.45\textwidth,
    legend style={
        at={(0.55,0.98)},
        anchor=north,
        legend columns=1,
        column sep=1.535ex,
        font=\Huge,
    },
    xlabel={\Huge Scale(B)},
    ylabel={\Huge Kurtosis},
    ylabel style={yshift=0.0em},
    xlabel style={yshift=0.0em},
    yticklabel style={
        font=\Huge
    },
    ytick={1,3,5,7,9},
    ymin=0, ymax=11,
    xmin=0, xmax=75,
    xtick={0,10,20,30,40,50,60,70},
    yticklabels={0,10,20,30,40,50,60,70}, % Y轴刻度标签
    xticklabel style={font=\Huge}
]

\addplot[orange!80,mark=triangle*,mark size=4pt,line width=3pt,mark options={fill=white,draw=orange}]
coordinates {(9,1) (34,1.34320503)};
\addlegendentry{\Huge Yi}

\addplot[green!80,mark=*,mark size=4pt,line width=3pt,mark options={fill=white,draw=green}]
coordinates {(3.82,1) (14,2.140025696)};
\addlegendentry{\Huge Phi}

\addplot[blue!60,mark=pentagon*,mark size=4pt,line width=3pt,mark options={fill=white,draw=blue}]
coordinates {(7,1) (14,1.348410468) (32,1.660721989) (72,5.139320896)};
\addlegendentry{\Huge Qwen}

\addplot[teal!70,mark=diamond*,mark size=5pt,line width=3pt,mark options={fill=white,draw=teal}]
coordinates {(8,1) (13,1.385530721) (70,1.800693756)};
\addlegendentry{\Huge LLaMA}

\addplot[red!70,mark=square*,mark size=4pt,line width=3pt,mark options={fill=white,draw=red}]
coordinates {(2,1) (7,1.822397447) (9,9.912905076)};
\addlegendentry{\Huge Gemma}

\end{axis}

\end{tikzpicture}

==> figures/test.tex <==


% Custom Kiviat diagram commands and definitions
\makeatletter
\def\tkz@KiviatGrad[#1](#2){% 
\begingroup
\pgfkeys{/kiviatgrad/.cd,
graduation distance= 0 pt,
prefix ={},
suffix={},
unity=1,
label precision/.store in=\gradlabel@precision,
label precision=0, % No decimal places
zero point/.store in=\tkz@grad@zero,
zero point=40 % Set zero point to 40
}
\pgfqkeys{/kiviatgrad}{#1}% 
\let\tikz@label@distance@tmp\tikz@label@distance
\global\let\tikz@label@distance\tkz@kiv@grad
 \foreach \nv in {1,...,\tkz@kiv@lattice}{
 \pgfmathsetmacro{\result}{35 + \nv * 5} % Start at 40 and increment by 5
 \protected@edef\tkz@kiv@gd{%
    \tkz@kiv@prefix%
    \pgfmathprintnumber[precision=\gradlabel@precision,fixed]{\result}%% used \pgfmathprintnumber instead of "\result\result"
    \tkz@kiv@suffix} 
    \path[/kiviatgrad/.cd,#1] (0:0)--(360/\tkz@kiv@radial*#2:\nv*\tkz@kiv@gap)
       node[label=(360/\tkz@kiv@radial*#2):\tiny\tkz@kiv@gd] {}; % added \tiny
      }
 \let\tikz@label@distance\tikz@label@distance@tmp  
\endgroup
}%
\makeatother

% Custom legend environment
\newenvironment{customlegend}[1][]{%
    \begingroup
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%

% Makes \addlegendimage available outside of an axis environment
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}

\definecolor{c1}{HTML}{CE93D8}
\definecolor{c2}{HTML}{ff8c1a}
\definecolor{c3}{HTML}{00aeef}
\definecolor{c4}{HTML}{B71C1C}
% Define global scale style
\tikzset{global scale/.style={
    scale=#1, % Set scaling factor
    every node/.append style={scale=#1} % Apply to every node
  }
}

\begin{tikzpicture}[
  label distance=13em, % Label distance
  global scale = 1, % Global scaling
  plot1/.style={ % Dataset 1 style
    thin, % Thin lines
    draw=c1, % Draw color red
    mark=square, % Marker shape square
   % fill=c1,
    mark options={
     ball color=c1, % Marker color red
     mark size=4pt % Marker size 4pt
    },
    opacity=.5 % Opacity 0.5
  },
  plot2/.style={ % Dataset 4 style
    thin,
    draw=c2,
    mark=triangle,
   % fill=c2,
    mark options={
      mark size=4pt,
      ball color=c2
    },
    opacity=.5
  },
  plot3/.style={ % Dataset 5 style
    thin,
    draw=c3,
    mark=square,
   % fill=c3,
    mark options={
      mark size=4pt,
      ball color=c3
    },
    opacity=.5
  },
  plot4/.style={ % Dataset 6 style
    thin,
    draw=c4,
    mark=triangle,
   % fill=c4,
    mark options={
      mark size=4pt,
      ball color=c4
    },
    opacity=.5
  }
]

\useasboundingbox (-25em,-5em) rectangle (10em,7em); % Set bounding box

\begin{scope}[scale=0.36,local bounding box=a,shift={(-12,0)}] % Set local scaling and position

% Define some macros for convenience
\newcommand\KivStep{0.1}
\pgfmathsetmacro\Unity{1/\KivStep}
\newcommand\zeroshift{20}

 \tkzKiviatDiagram[
   radial  style/.style ={-},
   rotate=90, 
   lattice style/.style ={black!30},
   step=\KivStep,
   gap=1,
   lattice=6,
]% 
{medmcqa,medqa,pubmedqa,careqa,AVG} % Define Kiviat diagram labels

 Draw dataset 1 Kiviat line
\tkzKiviatLine[
  plot1
](23.13889552,18.92380204,24.6,34.07400818,25.18417644)

Draw dataset 4 Kiviat line
 \tkzKiviatLine[
 plot2
 ](28.8764045,24.57973292,21.8,49.90748978,31.2909068)

 Draw dataset 5 Kiviat line
\tkzKiviatLine[
  plot3
 ](31.21922066,28.97879026,17.4,52.43373066,32.50793540)

 Draw dataset 6 Kiviat line
\tkzKiviatLine[
   plot4
 ](30.21515658,25.20816968,15.2,50.93933464,30.39066522)

% Draw graduation labels

\end{scope}

\begin{customlegend}[legend columns=2,legend style={draw=none,column sep=1ex,xshift=-8.5em,yshift=-9.5em},legend entries={model1,model 2,model 3,model4}]{(0em,-10em)}
    \addlegendimage{c1,fill=c1,mark=square,sharp plot}
    \addlegendimage{c2,fill=c2,mark=triangle,sharp plot}
    \addlegendimage{c3,fill=c3,mark=square,sharp plot}
    \addlegendimage{c4,fill=c4,mark=triangle,sharp plot}
\end{customlegend}

\end{tikzpicture}
